Eliza: A Web3 friendly AI Agent Operating System

AI Agent, powered by large language models (LLMs) as its cognitive core, is an intelligent agentic system capable of autonomously controlling and determining the execution paths under user's instructions. With the burst of capabilities of LLMs and various plugins, such as RAG, text-to-image/video/3D, etc., the potential of AI Agents has been vastly expanded, with their capabilities growing stronger by the day. However, at the intersection between AI and web3, there is currently no ideal agentic framework that can seamlessly integrate web3 applications into AI agent functionalities. In this paper, we propose Eliza, the first open-source web3-friendly Agentic framework that makes the deployment of web3 applications effortless. We emphasize that every aspect of Eliza is a regular Typescript program under the full control of its user, and it seamlessly integrates with web3 (i.e., reading and writing blockchain data, interacting with smart contracts, etc.). Furthermore, we show how stable performance is achieved through the pragmatic implementation of the key components of Eliza's runtime. Our code is publicly available at https://github.com/ai16z/eliza.

==> figures/tsne.tex <==
\begin{wrapfigure}{h}{0.32\linewidth}
    \vspace{-1.0em}
    \centering
    \includegraphics[width=0.9\linewidth]{images/tsne.png}
    \caption{TSNE visualization for pose distribution of RHD, FreiHAND, and \dataset.}
    \vspace{-2.0em}
\label{fig:tsne}
\end{wrapfigure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/ablation_accessories.tex <==
\begin{table}[h]
\vspace{-0.5em}
    \caption{Ablation study on training w/ and w/o \method's accessories.}
    \begin{center}
    % \resizebox{1.0\linewidth}{!}{
        \setlength{\aboverulesep}{0pt}
        \setlength{\belowrulesep}{0pt}
        \renewcommand{\arraystretch}{1}
        \begin{tabular}{c|cc|cc}
        \toprule
            \multirow{2}{*}{Method} & \multicolumn{2}{c}{Integral Pose \cite{sun2018integral}} & \multicolumn{2}{c}{CMR \cite{chen2021handmesh}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
            & w/o. Acs & w/. Acs & w/o. Acs & w/. Acs \\
        \midrule
            PA-MPJPE $\downarrow$ ($cm$) & 6.15 & 5.67 & 7.65 & 7.20 \\
            PA-MPVPE $\downarrow$ ($cm$) & -    & -    & 6.73 & 6.24 \\
        \bottomrule
        \end{tabular}
    % }
    \end{center}
    \label{table:ablation_accessories}
\end{table}

==> tables/benchmark.tex <==
\begin{table}[h]
\vspace{-0.5em}
\caption{3D hand pose / mesh reconstruction results on four learning-based methods.}
\label{tab:benchmark}
\centering
\begin{tabular}{c|c|c|c|c}
\toprule
 & Integral Pose \cite{sun2018integral} & RLE \cite{li2021rle} & CMR \cite{chen2021handmesh} & METRO \cite{lin2021metro} \\
\hline
PA-MPJPE $\downarrow$ ($cm$)  & \textbf{3.52}  & 4.45    & 4.84    & 3.96  \\
PA-MPVPE $\downarrow$ ($cm$)  & -   & -    & \textbf{3.46}    & 3.52   \\
\bottomrule
\end{tabular}
\end{table}

==> tables/cross_dataset.tex <==
\begin{table*}[h]
    \begin{center}
        \begin{minipage}[t]{0.47\textwidth}
        \caption{Cross-dataset evaluation on CMR (PA-MPJPE / PA-MPVPE ($cm$)).}\vspace{-2mm}
        \begin{center}
        \makeatletter\def\@captype{table}\makeatother
        \resizebox{1.0\linewidth}{!}{
            \begin{tabular}{l|ccc}
                \toprule
                \backslashbox{test}{train} & \freihand  & \dataset & Mixed \\
                \hline
                \freihand & 7.41 / 7.50 & 25.64 / 25.73 & \textbf{6.70} / \textbf{6.83} \\ 
                \dataset & 12.82 / 11.95 & 4.84 / 3.46 & 5.30 / 4.10 \\
                \bottomrule
            \end{tabular}
            }
        \end{center}
        \label{table:cmr_mix}
        \end{minipage}
        \quad\quad
        \begin{minipage}[t]{0.47\textwidth}
        \caption{Cross-dataset evaluation on METRO (PA-MPJPE / PA-MPVPE ($cm$)).}\vspace{-2mm}
        \begin{center}
            \resizebox{1.0\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
                \begin{tabular}{l|ccc}
                \toprule
                \backslashbox{test}{train} & \freihand & \dataset & Mixed \\
                \hline
                \freihand & 7.35 / 6.94 & 17.73 / 17.58 & \textbf{6.88} / \textbf{6.85} \\ 
                \dataset & 11.73 / 10.67 & 3.96 / 3.52 & \textbf{3.82} / 3.73 \\
                \bottomrule
            \end{tabular}
        }
        \end{center}

            \label{table:metro_mix}
        \end{minipage}
        ~~

    \end{center}
    % \vspace{-1.5em}
\end{table*}



==> tables/dataset_statistics.tex <==
\begin{table}[t]
\caption{Comparison among RGB-based 3D hand datasets. Note that syn indicates synthetic data, real indicates real captured data, and Tex. \& As. means the textures and accessories.}
\label{tab:dataset_stat}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
 & STB \cite{zhang20163d} & RHD \cite{zimmermann2017learning} & GANH. \cite{mueller2018ganerated} & FreiH. \cite{zimmermann2019freihand} & ObMan \cite{hasson2019obman} & InterH. \cite{moon2020interhand2} & \dataset (ours) \\
\hline
Type  & real & syn & syn & real & syn & real & syn \\
Size & 36K & 44K & 331K & 134K & 153K & 2.6M & 800K \\
Mesh & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark \\
Tex. \& As. & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/psedo-code.tex <==
\begin{figure}[H]
\begin{subfigure}[b]{0.64\linewidth}
\begin{algorithmic}[1]
	    \footnotesize
	    \ttfamily
	    \algrule
		\REQUIRE $W_\text{init}\in \mathbb{R}^{778 \times 16}, P_\text{init} \in \mathbb{R}^{778 \times 3 \times 135}, R_\text{init} \in \mathbb{R}^{778 \times 16}$
		\STATE $W_\text{final}$ = $\textbf{torch.\textcolor{blue}{zeros}}(842, 16)$
		\STATE $W_\text{final}[:778]$ = $W_\text{init}$ \STATE $W_\text{final}[778:842]$ = $W_\text{init}[777]$
		\STATE $P_\text{final}$ = $\textbf{torch.\textcolor{blue}{zeros}}(842, 3, 15)$
		\STATE $P_\text{final}[:778, :, :]$ = $P_\text{init}$
		\STATE $R_\text{final}$ = $\textbf{torch.\textcolor{blue}{zeros}}(842, 16)$
		\STATE $R_\text{final}[:778]$ = $R_\text{init}$
		\ENSURE  $W_\text{final}, P_\text{final}, R_\text{final}, \text{used for MANO's LBS}$
		\algrule
	\end{algorithmic}
	\caption{Pseudo code of alignment process}
	\label{arg:alignment}
\end{subfigure}
\hfill
\begin{subfigure}[][-10pt][b]{0.26\linewidth}
    \includegraphics[width=1.0\linewidth]{images/wrist.pdf}
    \caption{Wrist-enhanced MANO}
    \label{fig:wrist}
\end{subfigure}
\vspace{-1.0em}
\caption{\method hand parametric model.}
\end{figure}
\vspace{-1.0em}


==> tables/texture.tex <==
\begin{table}[t]
  \centering
  \adjustimage{width=7.6cm,valign=M}{images/texture.pdf}\qquad%
  \resizebox{0.25\linewidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Basic Texture  & Amount \\
    \midrule
    Bandage & 5 $\times$ 3  \\
    Palm prints & 10 $\times$ 3  \\
    Scars & 20 $\times$ 3  \\
    Tattoos & 20 $\times$ 3  \\
    Moles & 20 $\times$ 3  \\
    Nail colors & 20 $\times$ 3  \\
    \midrule
    Total & 285\\
    \\
    \toprule
    Accessories & Amount\\
    \midrule
    Rings  & 10 \\
    Watches  & 10 \\
    Bracelet  & 20 \\
    Gloves & 10 \\
    \midrule
    Total & 50\\
  \end{tabular}}
  \vspace{1em}
  \caption{Samples (left) and statistics (right) of \method's textures and accessories. All textures contain 3 basic skin tones: {\bf\textcolor{black}{dark}, \textcolor{brown}{brown}, \textcolor{pink}{light}}. Note that since above skin tones are represented as the same 2D UV map, it's relatively easy to extend them from other skin tone libraries.}
  \vspace{-2.0em}
  \label{tab:texture}
\end{table}
